Benign Oscillation of Stochastic Gradient Descent with Large Learning Rates

In this work, we theoretically investigate the generalization properties of neural networks (NN) trained by stochastic gradient descent (SGD) algorithm with large learning rates. Under such a training regime, our finding is that, the oscillation of the NN weights caused by the large learning rate SGD training turns out to be beneficial to the generalization of the NN, which potentially improves over the same NN trained by SGD with small learning rates that converges more smoothly. In view of this finding, we call such a phenomenon "benign oscillation". Our theory towards demystifying such a phenomenon builds upon the feature learning perspective of deep learning. Specifically, we consider a feature-noise data generation model that consists of (i) weak features which have a small $\ell_2$-norm and appear in each data point; (ii) strong features which have a larger $\ell_2$-norm but only appear in a certain fraction of all data points; and (iii) noise. We prove that NNs trained by oscillating SGD with a large learning rate can effectively learn the weak features in the presence of those strong features. In contrast, NNs trained by SGD with a small learning rate can only learn the strong features but makes little progress in learning the weak features. Consequently, when it comes to the new testing data which consist of only weak features, the NN trained by oscillating SGD with a large learning rate could still make correct predictions consistently, while the NN trained by small learning rate SGD fails. Our theory sheds light on how large learning rate training benefits the generalization of NNs. Experimental results demonstrate our finding on "benign oscillation".

==> tex/overview_of_analysis.tex <==
\section{Overview of Analysis}\label{sec: overview}

\textcolor{red}{I do not suggest to add this section in the main part, since the key intuition has been well justified in Section 3. Leave more space for discussions and figures.}
We define three important stopping times as following, for any $t_0\geq 0$,
\begin{align}
    T^{j,+}_{\mathbf{v}}(t_0) &= \inf_{t\geq t_0}\left\{t: \frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{j,r}^{(t)},j\mathbf{v}\rangle)> \delta/2\right\}, \\
    T^{j,-}_{\mathbf{v}}(t_0) &= \inf_{t\geq t_0}\left\{t: \frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{-j,r}^{(t)},j\mathbf{v}\rangle)> \delta/4\right\}, \\
     T_{\boldsymbol{\xi}}(t_0) &= \inf_{t\geq t_0}\left\{t: \exists i\in[n],\left|\frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{j,r}^{(t)},\boldsymbol{\xi}_i\rangle) - \sigma(\langle\mathbf{w}_{-j,r}^{(t)},\boldsymbol{\xi}_i\rangle)\right|> \delta/4\right.\\
     &\qquad\left.\vee\,\,\,\exists i\in\mathcal{W},\left|\frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{j,r}^{(t)},\widetilde{\boldsymbol{\xi}}_i\rangle) - \sigma(\langle\mathbf{w}_{-j,r}^{(t)},\widetilde{\boldsymbol{\xi}}_i\rangle)\right|> \delta/4\right\}. 
\end{align}
We recap that $\mathcal{W}$ denotes the index set of weak data, and $\widetilde{\boldsymbol{\xi}}_i$ denotes the Gaussian noise appearing on the lacking strong signal patch for those weak data.
Note that $T^{j,+}_{\mathbf{v}}$, $T^{j,-}_{\mathbf{v}}$, $T_{\boldsymbol{\xi}}\in[t_0,+\infty]$.
We define $T_{\max}^j(t_0) = \min\{T^{j,+}_{\mathbf{v}}(t_0), T^{j,-}_{\mathbf{v}}(t_0), T_{\boldsymbol{\xi}}(t_0)\} - 1$. 
% Then by definition \eqref{eq: event} we know that event $\mathcal{E}_j^{T_{\max}^j}$ holds.

\begin{proposition}[Linear accumulation of oscillation]\label{prop: linear accumulation}
    Under Assumptions \ref{ass: conditions} and \ref{ass: oscillation}, with probability at least $1-1/\mathrm{poly}(d)$, it holds that for any $j\in\{\pm 1\}$ and $t_0\leq t_1\leq t_2\leq T_{\max}^j(t_0)$ that 
    \begin{align}
        \sum_{\substack{s=t_1 \\ y_{i_s} = j}}^{t_2} 1 - y_{i_s}f(\mathbf{x}_{i_s};\mathbf{W}^{(s)}) \geq \frac{\delta}{16}\cdot\big(1 - (1-\delta/4 )^{\frac{1}{2}}\big) \cdot(t_2 - t_1 + 1) - \frac{m\textcolor{purple}{(1.05\cdot(1+\delta))^{\frac{1}{2}}}}{2\eta\|\mathbf{u}\|_2^2(1- \delta/4)^{\frac{1}{2}}},
    \end{align}
    where $\delta$ is specified in Assumption \ref{ass: oscillation}.
\end{proposition}
\begin{proof}[Proof of Proposition \ref{prop: linear accumulation}]
    See Appendix \ref{subsec: proof linear accumulation} for a detailed proof.
\end{proof}

\begin{proposition}[Weak signal learning \uppercase\expandafter{\romannumeral1}]\label{prop: signal learning 1}
    Under Assumptions \ref{ass: conditions} and \ref{ass: oscillation}, then with probability at least $1-1/\mathrm{poly}(d)$, it holds for any $t_0\leq t\leq T_{\max}^j(t_0) $, $j\in\{\pm 1\}$, and $r\in\mathcal{C}_{j,+}^{(t)}$ that 
    \begin{align}
        \dotp{\wb_{j,r}^{(t+1)}}{j\vb} &\geq \dotp{\wb_{j,r}^{(t_0)}}{j\vb} \!\cdot\!\exp\left\{\frac{\eta\|\mathbf{v}\|_2^2}{32m}\!\cdot\!\big(\delta - \delta(1-\delta/4 )^{\frac{1}{2}}\big) \!\cdot\!(t - t_0 + 1) - \frac{\|\mathbf{v}\|_2^2\textcolor{purple}{(1.05(1+\delta))^{\frac{1}{2}}}}{\|\mathbf{u}\|_2^2(1- \delta/4)^{\frac{1}{2}}}\right\}.
    \end{align}
    % and $\widetilde{T}^+_{(\mathbf{v})} = \widetilde{\Theta}(m\cdot\eta^{-1}\cdot(\|\mathbf{v}\|_2^{-2} + \|\mathbf{u}\|_2^{-2}))$.
\end{proposition}
\vspace{-6mm}
\begin{proof}[Proof of Proposition \ref{prop: signal learning 1}]
    See Appendix~\ref{subsec: proof signal learning 1} for a detailed proof.
\end{proof}



\begin{proposition}[Weak signal learning \uppercase\expandafter{\romannumeral2}]\label{prop: signal learning 2}
Under Assumptions \ref{ass: conditions} and \ref{ass: oscillation}, then with probability at least $1-1/\mathrm{poly}(d)$, it holds for any $t_0\leq t< T_{\max}^j(t_0)$ and $j\in\{\pm 1\}$ that 
\begin{align}
    -\langle \mathbf{w}_{-j,r}^{(t)},j\mathbf{v}\rangle \geq - 3\cdot \langle \mathbf{w}_{-j,r}^{(t_0)},j\mathbf{v}\rangle,\quad \forall r\notin\mathcal{C}_{-j,+}^{(t)}.
\end{align}
\end{proposition}

\begin{proof}[Proof of Proposition \ref{prop: signal learning 2}]
    See Appendix~\ref{subsec: proof signal learning 2} for a detailed proof.
\end{proof}

% \textcolor{gray}{\begin{proposition}[Signal learning \uppercase\expandafter{\romannumeral2}]\label{prop: signal learning 2}
% Under Assumptions \ref{ass: conditions}, \ref{ass: boundedness}, and \ref{ass: oscillation}, then with probability at least $1-1/\mathrm{poly}(d)$, it holds for any $0\leq t_0< T_{\max}^j - \widetilde{T}_{(\mathbf{v})}^-$ and $j\in\{\pm 1\}$ that 
% \begin{align}
%     -\langle \mathbf{w}_{-j,r}^{(t_0+\widetilde{T}^+_{(\mathbf{v})})},j\mathbf{v}\rangle \geq - \langle \mathbf{w}_{-j,r}^{(t_0)},j\mathbf{v}\rangle\cdot(1-\epsilon),\quad \forall r\notin\mathcal{C}_{-j,+}^{(t)},
% \end{align}
% where $\epsilon = \delta\cdot(1 - (1-\delta/2+\munderbar{c}^2)^{\frac{1}{2}})/28$ and $\widetilde{T}^-_{(\mathbf{v})} = \widetilde{T}^+_{(\mathbf{v})} = \widetilde{\Theta}(m\cdot\eta^{-1}\cdot(\|\mathbf{v}\|_2^{-2} + \|\mathbf{u}\|_2^{-2}))$.
% \end{proposition}}

For simplicity, we define the maximum absolute value of the noise inner products over data as 
\begin{align}
    \Upsilon^{(t)} = \max_{j\in\{\pm 1\}}\left\{\max_{i\in[n]}\left|\langle \mathbf{w}_{j,r}^{(t)},\boldsymbol{\xi}_i\rangle\right|,\max_{i\in\mathcal{W}}\left|\langle \mathbf{w}_{j,r}^{(t)},\widetilde{\boldsymbol{\xi}}_i\rangle\right|\right\}
\end{align}

\begin{proposition}[Noise memorization]\label{prop: noise memorization}
    Under Assumptions \ref{ass: conditions} and \ref{ass: oscillation}, then with probability at least $1-1/\mathrm{poly}(d)$, it holds for any $t_0\leq t_1  \leq T_{\boldsymbol{\xi}}(t_0) - \widetilde{T}_{(\boldsymbol{\xi})}$, and $j\in\{\pm 1\}$ that 
    \begin{align}
        \Upsilon^{(t)}\leq \Upsilon^{(t_1)}\cdot(1+\epsilon),\quad \forall r\in[m],\quad \forall t_1\leq t\leq t_1+\widetilde{T}_{(\boldsymbol{\xi})}
    \end{align}
    where $\widetilde{T}_{(\boldsymbol{\xi})} = \widetilde{\Theta}(mn\cdot\eta^{-1}\cdot\epsilon\cdot(1+\epsilon)^{-1}\cdot(\sigma_p^2d)^{-1})$.
\end{proposition}

\begin{proof}[Proof of Proposition \ref{prop: noise memorization}]
    See Appendix~\ref{subsec: proof noise memorization} for a detailed proof.
\end{proof}

With Propositions~\ref{prop: signal learning 1}, \ref{prop: signal learning 2}, and \ref{prop: noise memorization}, we are ready to prove Theorem~\ref{thm: main}.
Let's start from step $t=0$.
% Consider by Proposition~\ref{prop: signal learning 1}, we know that for any $l\in\mathbb{N}$ such that $l\widetilde{T}_{(\mathbf{v})}^+ \leq T_{\max}^j$, 
% \begin{align}
%     \frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{j,r}^{(l\widetilde{T}_{(\mathbf{v})}^+)},j\mathbf{u}\rangle) = \frac{1}{m}\sum_{r\mathcal{C}_{j,+}^{(0)}}\sigma(\langle\mathbf{w}_{j,r}^{(l\widetilde{T}_{(\mathbf{v})}^+)}, j\mathbf{u}\rangle)  \geq (1+\epsilon)^{2l}\sum_{r\mathcal{C}_{j,+}^{(0)}}\sigma(\langle\mathbf{w}_{j,r}^{(0)}, j\mathbf{u}\rangle),
% \end{align}
% Consequently, we can see that $T_{\max}^j = \min\{T^{j,+}_{\mathbf{(v)}}, T^{j,-}_{\mathbf{(v)}}, T_{(\boldsymbol{\xi})}^{j}\} - 1$ satisfies 
% \begin{align}
%     T_{\max}^j \leq l^{\ast}\widetilde{T}_{(\mathbf{v})}^+,\quad l^{\ast} = \log\left(\frac{1}{4}\delta m/ \sum_{r\in[m]}\sigma(\langle\mathbf{w}_{j,r}^{(0)}, j\mathbf{u}\rangle)\right) / \log(1+\epsilon),
% \end{align}
% since otherwise $\frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{j,r}^{(l^{\ast}\widetilde{T}_{(\mathbf{v})}^+)},j\mathbf{u}\rangle) \geq \delta/4$ which contradicts the definition of $T_{\max}^j$.
% In the sequel, we are going to show that both $T^{j,-}_{\mathbf{(v)}}$ and $T^{j}_{(\boldsymbol{\xi})}$ is no smaller than $T_{(\mathbf{v})}^{j,+}$, further indicating that $T_{\max}^j = T^{j,+}_{\mathbf{(v)}} - 1$ and finishing the proof of Theorem \ref{thm: main}.

% \textcolor{blue}{For $T^{j,-}_{\mathbf{(v)}}$, use Proposition \ref{prop: signal learning 2}; for $T^{j}_{(\boldsymbol{\xi})}$, use Proposition \ref{prop: noise memorization}.}

% In fact, by Proposition \ref{prop: signal learning 2}, which is stronger than what we need, we can simply obtain that 
% \begin{align}
%     \frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{-j,r}^{(l^{\ast}\widetilde{T}_{(\mathbf{v})}^+)},j\mathbf{v}\rangle) \leq \frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{-j,r}^{(0)},j\mathbf{v}\rangle) \leq \widetilde{\mathcal{O}}(\sigma_0^2\|\mathbf{v}\|_2^2) \leq \frac{\delta}{8},
% \end{align}
% and by Proposition \ref{prop: noise memorization}, we can also obtain that for any $i\in[n]$,
% \begin{align}
%     \left|\frac{1}{m}\sum_{r\in[m]}\sigma(\langle\mathbf{w}_{j,r}^{(l^{\ast}\widetilde{T}_{(\mathbf{v})}^+))},\boldsymbol{\xi}_i\rangle) - \sigma(\langle\mathbf{w}_{j,r}^{(l^{\ast}\widetilde{T}_{(\mathbf{v})}^+)},\boldsymbol{\xi}_i\rangle)\right|
% \end{align}
